CovarianceNet: Conditional Generative Model for Correct Covariance Prediction in Human Motion Prediction

The correct characterization of uncertainty when predicting human motion is equally important as the accuracy of this prediction. We present a new method to correctly predict the uncertainty associated with the predicted distribution of future trajectories. Our approach, CovariaceNet, is based on a Conditional Generative Model with Gaussian latent variables in order to predict the parameters of a bi-variate Gaussian distribution. The combination of CovarianceNet with a motion prediction model results in a hybrid approach that outputs a uni-modal distribution. We will show how some state of the art methods in motion prediction become overconfident when predicting uncertainty, according to our proposed metric and validated in the ETH data-set \cite{pellegrini2009you}. CovarianceNet correctly predicts uncertainty, which makes our method suitable for applications that use predicted distributions, e.g., planning or decision making.

==> plan.tex <==
\section{PLAN}

\begin{itemize}
  \item Abstract
  \item Introduction
  \item Related work
  \item Problem formulation (optional)
  \item Proposed Method
  \item Experiments (optional)
  \item Conclusion
  \item Bibliography
\end{itemize}


\subsection{Long story short}
\subsubsection{Abstract}
We presenting new approach to human MP, with focusing on accurately predicting uncertainties
\subsubsection{Intro}
Story why human MP \& accurately predicting uncertainties is important. 
In this work we are interested in developing ...
In this work we present "NAME" an open and extensible approach for ...

\begin{itemize}
    \item In this work, we aim to tackle the task of human trajectory prediction ...
    \item SFM + COV\_NET + Maybe GOAL\_PRED  = result
    \item architecture
    \item losses

\end{itemize}


\subsubsection{Experiments}
\begin{itemize}
    \item Datasets
    \item Metrics
    \item Quantitative Results
\end{itemize}

\subsubsection{Conclusion}
\begin{itemize}
    \item In this work we present ... 
    \item We show that ...
    \item Further, we perform extensive ablations on our design choices
    \item Finally, we benchmark XXX across multiple datasets including
\end{itemize}


\newpage
\section{skeleton draft}
\begin{equation}
    trajectory^{n}_p = { p^{n}_t = (x^n_t,y^n_t) | t \in {1, ..., T_{p}}} 
\end{equation}
where $(x^n_t, y^n_t)$ are random variables s describing the probability distribution of the location of pedestrian n at time t, in the 2D space.

Model is trained to minimize the negative log-likelihood and KL div (CVAE architecture), which defined as:

\begin{align*}
    &L^n_{nll}(W) = -\sum^{T_p}_{t=1}log(P(p^{n}_t| \mu, \sigma,\rho))
    \\
    &L^n_{kl} = D_{kl}(q_\phi(z | x,y) || p_{\theta}(z|x))
    \\
    &Loss = \alpha  L^n_{nll}(W) + L^n_{kl}
\end{align*}

A tentative loss function including the average of the indicator function counting the number of times we are in the 1,3-$\sigma$ interval.
This is similar to differential RANSAC
\begin{align}
    L = | E\{ \mathcal{U}( d_{MH}(e) <  1 )\} - 0.39| +| E\{ U ( d_{MH}(e)  < 3 )\} - 0.98|
\end{align}


Mahalanobis distance 
\begin{align*}
    D_M(x) = \sqrt{(x - \mu)^T S^{-1}(x - \mu)}
\end{align*}


1-3 sigma rules

\begin{align*}
    Pr(\mu- 1\sigma \leq X \leq \mu + 1\sigma) \approx 0.6827 (1D-case)
    \\
    Pr(\mu- 3\sigma \leq X \leq \mu + 3\sigma) \approx 0.9973 (1D-case)
\end{align*}

% TODO add others

% \begin{figure}[h]%
%     \centering
%     \subfloat[\centering label 1]{{\includegraphics[width=7cm]{img/before_calib_1.png} }}
%     \hfill
%     \subfloat[\centering label 2]{{\includegraphics[width=7cm]{img/after_calib_1.png} }}
%     \caption{calibration effect}%
%     \label{fig:example}%
% \end{figure}




\begin{figure}[h]
    \includegraphics[width=8cm]{img/visualizations.png}
    \caption{An example of trajectory prediction visualization}
\end{figure}


\newpage




==> references.tex <==


\begin{thebibliography}{99}

\bibitem{c1} Postnikov, A., Gamayunov, A., Ferrer, G. (2020). HSFM-$\Sigma $ nn: Combining a Feedforward Motion Prediction Network and Covariance Prediction. arXiv preprint arXiv:2009.04299.
\bibitem{c2} Mehta, D., Ferrer, G., Olson, E. (2018, May). Backprop-MPDM: Faster risk-aware policy evaluation through efficient gradient optimization. In 2018 IEEE International Conference on Robotics and Automation (ICRA) (pp. 1740-1746). IEEE.
% \bibitem{sfm} Helbing, D., Molnar, P. (1995). Social force model for pedestrian dynamics. Physical review E, 51(5), 4282.

% \bibitem{hsfm} Farina, F., Fontanelli, D., Garulli, A., Giannitrapani, A., Prattichizzo, D. (2017). Walking ahead: The headed social force model. PloS one, 12(1), e0169734.
% \bibitem{trajectron++} Salzmann, T., Ivanovic, B., Chakravarty, P., Pavone, M. (2020). Trajectron++: Multi-agent generative trajectory forecasting with heterogeneous data for control. arXiv preprint arXiv:2001.03093.
% \bibitem{social-lstm} Alahi, A., Goel, K., Ramanathan, V., Robicquet, A., Fei-Fei, L., Savarese, S. (2016). Social lstm: Human trajectory prediction in crowded spaces. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 961-971).
% \bibitem{social-pooling}Messaoud, Kaouther, et al. "Non-local social pooling for vehicle trajectory prediction." 2019 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2019.

% \bibitem{CVAE} Sohn, Kihyuk, Honglak Lee, and Xinchen Yan. "Learning structured output representation using deep conditional generative models." Advances in neural information processing systems. 2015.

% \bibitem{GANS} Goodfellow, Ian, et al. "Generative adversarial nets." Advances in neural information processing systems. 2014.
\bibitem{c7} Giuliari, F., Hasan, I., Cristani, M., Galasso, F. (2020). Transformer Networks for Trajectory Forecasting. arXiv preprint arXiv:2003.08111.
\bibitem{c8} Mohamed, A., Qian, K., Elhoseiny, M., Claudel, C. (2020). Social-STGCNN: A Social Spatio-Temporal Graph Convolutional Neural Network for Human Trajectory Prediction. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 14424-14432).
\bibitem{mcanaliz} Janssen, H. (2013). Monte-Carlo based uncertainty analysis: Sampling efficiency and sampling convergence. Reliability Engineering \& System Safety, 109, 123-132.



% \bibitem{theDestination} Mangalam, K., Girase, H., Agarwal, S., Lee, K. H., Adeli, E., Malik, J., Gaidon, A. (2020). It Is Not the Journey but the Destination: Endpoint Conditioned Trajectory Prediction. arXiv preprint arXiv:2004.02025.
\bibitem{c10} Yi, S., Li, H., Wang, X. (2016, October). Pedestrian behavior understanding and prediction with deep neural networks. In Eu
\bibitem{c11} Zhang, P., Ouyang, W., Zhang, P., Xue, J., Zheng, N. (2019). Sr-lstm: State refinement for lstm towards pedestrian trajectory prediction. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 12085-12094).
\bibitem{c12} Gupta, A., Johnson, J., Fei-Fei, L., Savarese, S., Alahi, A. (2018). Social gan: Socially acceptable trajectories with generative adversarial networks. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 2255-2264).
\bibitem{c13} Abdelaziz, A. H., Watanabe, S., Hershey, J. R., Vincent, E., Kolossa, D. (2015, September). Uncertainty propagation through deep neural networks.
\bibitem{c14} Rehder, Eike, and Horst Kloeden. ”Goal-directed pedestrian prediction.” Proceedings of the IEEE International Conference on Computer Vision Workshops. 2015.
\bibitem{c15} Fernando, Tharindu, et al. ”Neighbourhood context embeddings in deep inverse reinforcement learning for predicting pedestrian motion over long time horizons.” Proceedings of the IEEE International Conference on Computer Vision Workshops. 2019.
\bibitem{c16} Becker, S., Hug, R., H¨ubner, W., Arens, M.: An evaluation of trajectory prediction approaches and notes on the trajnet benchmark. arXiv preprint arXiv:1805.07663 (2018)
\bibitem{c17} Deo, N., Trivedi, M.M.: Trajectory forecasts in unknown environments conditioned on grid-based plans. arXiv preprint arXiv:2001.00735 (2020)
\bibitem{c18} Hang Su, Jun Zhu, Y.D.B.Z.: Forecast the plausible paths in crowd scenes. In: IJCAI (2017)
\bibitem{c19} Ivanovic, B., Pavone, M.: The trajectron: Probabilistic multi-agent trajectory modeling with dynamic spatiotemporal graphs. In: Proceedings of the IEEE International Conference on Computer Vision. pp. 2375–2384 (2019)
\bibitem{c20} Zhang, P., Ouyang, W., Zhang, P., Xue, J., Zheng, N. (2019). Sr-lstm: State refinement for lstm towards pedestrian trajectory prediction. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 12085-12094).
\bibitem{c22} Ellis, D., Sommerlade, E., Reid, I. (2009, September). Modelling pedestrian trajectory patterns with gaussian processes. In 2009 IEEE 12th International Conference on Computer Vision Workshops, ICCV Workshops (pp. 1229-1234). IEEE.
\bibitem{c23} Bao, J., Chen, D., Wen, F., Li, H., Hua, G. (2017). CVAE-GAN: fine-grained image generation through asymmetric training. In Proceedings of the IEEE international conference on computer vision (pp. 2745-2754).
\bibitem{c24} Guo, C., Pleiss, G., Sun, Y., Weinberger, K. Q. (2017). On calibration of modern neural networks. arXiv preprint arXiv:1706.04599.

\bibitem{mah}De Maesschalck, Roy, Delphine Jouan-Rimbaud, and Désiré L. Massart. "The mahalanobis distance." Chemometrics and intelligent laboratory systems 50.1 (2000): 1-18.
\bibitem{eth}Pellegrini, S., Ess, A., Schindler, K., Gool, L.V.: You’ll never walk alone: Modeling
social behavior for multi-target tracking. In: IEEE Int. Conf. on Computer Vision
(2009)

% \bibitem{Bahdanau}Bahdanau, Dzmitry, Kyunghyun Cho, and Yoshua Bengio. "Neural machine translation by jointly learning to align and translate." arXiv preprint arXiv:1409.0473 (2014).

\end{thebibliography}
